An Information-Theoretic Approach for Detecting Edits in AI-Generated Text

We propose a method to determine whether a given article was written entirely by a generative language model or perhaps contains edits by a different author, possibly a human. Our process involves multiple tests for the origin of individual sentences or other pieces of text and combining these tests using a method that is sensitive to rare alternatives, i.e., non-null effects are few and scattered across the text in unknown locations. Interestingly, this method also identifies pieces of text suspected to contain edits. We demonstrate the effectiveness of the method in detecting edits through extensive evaluations using real data and provide an information-theoretic analysis of the factors affecting its success. In particular, we discuss optimality properties under a theoretical framework for text editing saying that sentences are generated mainly by the language model, except perhaps for a few sentences that might have originated via a different mechanism. Our analysis raises several interesting research questions at the intersection of information theory and data science.

==> media_summary.tex <==
% The Media Summary should be written in plain language to highlight the key messages of
% the article, in ways that can be understood by the general public and cited by the media 
% directly and accurately. It therefore should avoid technical terms or language designed for
% academic communications. It should not exceed 400 words, and more succinct, the better.
Suppose that an article that was initially written by a generative language model (GLM) such as ChatGPT undergoes relatively minor changes. For example, a human editor adds, removes, or rephrases certain sentences. This
work aims to detect the presence of such edits and identify the edited parts if they exist.

The popularity of GLM-assisted tools for writing raises tremendous interest in detecting GLM text for several reasons, e.g., maintaining trust and ethical standards in authored material. The scenario we consider corresponds to a particularly challenging situation within this context because human edits, if present, are scattered across the article in some locations that are unknown in advance. 
%
Furthermore, edits are associated with relatively short pieces of text like sentences. Given the similarity between text generated by modern GLMs and human writing, identifying human involvement over such brief excerpts is arguably challenging, if not impossible. 
%
Metaphorically, we seek to detect needles in a haystack, without knowing how many needles there are, if any. These challenges are well-understood in the context of multiple comparisons and rare and weak signal detection in statistics. In this work, we present an approach to detect and identify edits in text that adapts tools from these domains. We showcase the effectiveness of our approach in various realistic scenarios using extensive evaluation, conduct a mathematical analysis to illustrate both its efficacy and limitations, and suggest potential avenues for improvement based on our findings.
